TeleLoRA: Teleporting Model-Specific Alignment Across LLMs

Mitigating Trojans in Large Language Models (LLMs) is one of many tasks where alignment data is LLM specific, as different LLMs have different Trojan triggers and trigger behaviors to be removed. In this paper, we introduce TeleLoRA (Teleporting Low-Rank Adaptation), a novel framework that synergizes model-specific alignment data across multiple LLMs to enable zero-shot Trojan mitigation on unseen LLMs without alignment data. TeleLoRA learns a unified generator of LoRA adapter weights by leveraging local activation information across multiple LLMs. This generator is designed to be permutation symmetric to generalize across models with different architectures and sizes. We optimize the model design for memory efficiency, making it feasible to learn with large-scale LLMs with minimal computational resources. Experiments on LLM Trojan mitigation benchmarks demonstrate that TeleLoRA effectively reduces attack success rates while preserving the benign performance of the models.

==> einnet.tex <==

\section{LLMs used for jailbreak study}
Seen LLMs: 
1) google/gemma-2-2b-it,
2) meta-llama/Llama-3.1-8B-Instruct,
3) google/gemma-2b-it,
4) meta-llama/Llama-3.2-3B-Instruct,
5) meta-llama/Llama-3.2-1B-Instruct,
6) microsoft/Phi-3.5-mini-instruct,
7) Qwen/Qwen2.5-1.5B-Instruct,
8) Qwen/Qwen2.5-3B-Instruct.



\section{Appendix: Permutation Symmetric Neural Networks}


Our approach analyzes the parameter sharing pattern induced by permutation symmetry in the Taylor series of a function, leveraging the null-space method from \cite{finzi2021practical}. We find that einsum operations are the fundamental building blocks needed for building high-order permutation invariant networks. We propose a network architecture that interleaves MLPs with einsum pooling operations for building generic permutation symmetric neural networks. Finally, we demonstrate the flexibility of permutation symmetric neural networks in the design of Trojan detection classifiers, ingesting weight matrices, neural activations and confusion matrices as features for Trojan detection. 


We first introduce the theoretical approach of using Taylor series to parameterize permutation symmetric functions. And then, we introduce our design of practical permutation symmetric neural networks guided by theory. Finally, we introduce how such a network can be applied to Trojan detection.


\subsection{Paramterizing Symmetric Functions in Taylor Series}

We introduce a simple yet general Taylor series-based view necessary for studying complex symmetry patterns. Specifically, we enable efficient universal learners -- that can represent any such invariant or equivariant functions. The general idea is similar to parallel works Equivariant Multilayer Perceptrons (EMLP)~\cite{finzi2021practical}, universal equivariant MLPs~\cite{ravanbakhsh2020universal}, Equivariant Polynomial layers\cite{puny2023equivariant} as well as many others, but our approach adds further simplifications to focus on parameter count and compute efficiency. 

Given the desired input-output shapes and symmetry constraints, we would proceed with the following steps: 
1) Express a general function that matches the input-output shapes in Taylor series form.
2) Map the symmetry constraints into equations about the Taylor series coefficients.
3) Solve the equations for free parameters and the parameter sharing patterns, and parameterize the function using the free parameters.
4) Simplify the parameterization for efficient computation.

Let us use 1D permutation invariance as an example.

Let\'s say we want to make a function 

\begin{align*}
y=f\left( \begin{bmatrix}x_{0} & x_{1} & x_{2}\end{bmatrix} \right)
\end{align*}

invariant to permutation of $x_0$, $x_1$, $x_2$.

Consider the Taylor series

\begin{align*}
f & \left( \begin{bmatrix}x_{0} & x_{1} & x_{2}\end{bmatrix} \right) \\
= & a + 
\begin{bmatrix} b_0 & b_1 & b_2\end{bmatrix} 
\begin{bmatrix} x_0 \\ x_1 \\ x_2 \end{bmatrix} +
\begin{bmatrix} x_0 & x_{1} & x_{2}\end{bmatrix}
\begin{bmatrix} 
    c_{00} & c_{01} & c_{02}\\
    c_{10} & c_{11} & c_{12}\\
    c_{20} & c_{21} & c_{22}
\end{bmatrix} 
\begin{bmatrix} x_{0} \\ x_{1} \\ x_{2} \end{bmatrix}
+ \ldots
\end{align*}

Since we want $f(\cdot)$ to be invariant to any permutation matrix $P$, the invariant constraint says 

\begin{align*}
f\left(\begin{bmatrix}x_{0} \\ x_{1} \\ x_{2}\end{bmatrix}\right)=f\left(
    \begin{bmatrix} 
      &   &  \\
      & P &  \\
      &   &  
    \end{bmatrix} 
    \begin{bmatrix}x_{0} \\ x_{1} \\ x_{2}\end{bmatrix}\right)
\end{align*}

For our Taylor series form, because of the uniqueness of Taylor series, all order-k coefficients on the left hand side need to match the corresponding order-k coefficients on the right hand side. That is for any permutation matrix $P$ we have


\begin{align*}
a = & a \\
\begin{bmatrix} b_0 & b_1 & b_2\end{bmatrix}  = &
\begin{bmatrix} b_0 & b_1 & b_2\end{bmatrix} 
    \begin{bmatrix} 
      &   &  \\
      & P &  \\
      &   &  
    \end{bmatrix} 
\\
\begin{bmatrix} 
    c_{00} & c_{01} & c_{02}\\
    c_{10} & c_{11} & c_{12}\\
    c_{20} & c_{21} & c_{22}
\end{bmatrix} 
=& 
\begin{bmatrix} 
    &   &  \\
    & P^T &  \\
    &   &  
\end{bmatrix} 
\begin{bmatrix} 
    c_{00} & c_{01} & c_{02}\\
    c_{10} & c_{11} & c_{12}\\
    c_{20} & c_{21} & c_{22}
\end{bmatrix} 
    \begin{bmatrix} 
      &   &  \\
      & P &  \\
      &   &  
    \end{bmatrix} \\
& \ldots
\end{align*}


These equations are all linear equations about coefficients $a$, $b_i$ and $c_{ij}$. So we can just enumerate all $P$ to get all the equations, and then solve them. For $b_i$ for example, enumerating different permutations $P$ would give

\begin{align*}
\begin{bmatrix} b_0 \\ b_1 \\ b_2\end{bmatrix}  = 
\begin{bmatrix} b_0 \\ b_2 \\ b_1\end{bmatrix}  = 
\begin{bmatrix} b_1 \\ b_0 \\ b_2\end{bmatrix}  = 
\begin{bmatrix} b_1 \\ b_2 \\ b_0\end{bmatrix}  = 
\begin{bmatrix} b_2 \\ b_0 \\ b_1\end{bmatrix}  = 
\begin{bmatrix} b_2 \\ b_1 \\ b_0\end{bmatrix} 
\end{align*}

That is more than enough to say $b_0=b_1=b_2$. So the order-1 term has only 1 degree of freedom.

For $c_i$ there are more equations, but it turns out that solving the equations across all permutations would yield 
$c_{00}=c_{11}=c_{22}$$ and $$c_{01}=c_{10}=c_{10}=c_{12}=c_{20}=c_{21}$. So the order 2 term has 2 degrees of freedom, one for the diagonal and one for everywhere else.

Applying what we have learned, we can now write

\begin{align*}
y=&f\left( \begin{bmatrix}x_{0} & x_{1} & x_{2}\end{bmatrix} \right)\\
= & a + 
\begin{bmatrix} b & b & b\end{bmatrix} 
\begin{bmatrix} x_0 \\ x_1 \\ x_2 \end{bmatrix} +
\begin{bmatrix} x_0 & x_{1} & x_{2}\end{bmatrix}
\begin{bmatrix} 
    c_{0} & c_{1} & c_{1}\\
    c_{1} & c_{0} & c_{1}\\
    c_{1} & c_{1} & c_{0}
\end{bmatrix} 
\begin{bmatrix} x_{0} \\ x_{1} \\ x_{2} \end{bmatrix}
+ \ldots
\end{align*}


For a total of 4 free parameters up to order 2, instead of 13 free parameters without the invariance constraint. More generally, for $N$ inputs, we still only need 4 parameters to express any permutation invariant function, whereas a non-invariant function needs $N^2+N+1$ parameters. In practice, parameterizing with symmetry often \textbf{reduces parameter count} exponentially. 

We can further simplify by focusing on the free parameters

\begin{align*}
y=&f\left( \begin{bmatrix}x_{0} & x_{1} & x_{2}\end{bmatrix} \right)\\
= & a + b \sum_i x_i + (c_0-c_1) \sum_i x_i^2 + c_1 \sum_{i} \sum_{j} x_i x_j + \ldots \\
= & a + b \sum_i x_i + (c_0-c_1) \sum_i x_i^2 + c_1 (\sum_{i}x_i )^2 + \ldots
\end{align*}

An important effect of this simplification is \textbf{reduced compute}. It now requires $O(N)$ compute for $N$ inputs instead of $O(N^2)$ for order-2.  

In math terms, the number of free parameters is the dimensionality of the null space of the symmetry equations. The free parameters can be numerically solved from the basis of this null space. But note that as the basis is often not unique, numerical solutions can vary by a linear combination and therefore may not be compute-optimal, so further simplification is still needed.

Although we didn't unroll order-3 and higher terms because they are difficult to visualize, they can still be analyzed with the same approach. Just imagine a cube or a hypercube of parameters, apply the symmetry transformations simultaneously along all dimensions and solve for the parameter sharing pattern.



In this section, we have learned that

1) Symmetry constraints reduce the number of free parameters.

2) A Taylor-series technique can be used to parameterize symmetric functions.

3) Different symmetries can have different impacts on degrees of freedom.

4) Certain parameterizations can reduce compute exponentially.

5) Parameterization of equivariant functions are tied to parameterization of invariant functions

6) Permutation invariant and equivariant functions can be parameterized solely using tensor contraction terms.


A Taylor series parameterization is sound in theory. In practice however, functions compound and high order interactions are common. Taylor series often provides too little relevant capacity and too much irrelevant capacity to be useful. Engineering is key in the journey to create universal learners of symmetric functions. In the next section, we'll focus on permutation symmetry and design a family of practical invariant and equivariant networks for various flavors of permutation symmetry.

\subsection{Engineering a Network with Permutation Symmetry}

From matrices to sets to symbolic processing, permutation symmetry is found in many problems and requires extra attention during modeling. When handled properly however, permutation symmetry is also a blessing. As we have learned in the previous section, if parameterized properly, permutation symmetry has the potential to exponentially reduce parameter count and compute for highly efficient learning. At the other end of the spectrum, reciting the success recipe of deep learning, we can scale the latent dimension and stack equivariant layers to create exponentially more expressive networks at the same parameter count and compute as a regular network.


Devil's in the details, in this section we'll walk through the design of permutation symmetric neural networks for various types of permutation symmetry.


There are many places where you'll see permutation symmetry and they often come in different forms. So we'll first start from a summary of common types of permutation symmetry, and then the design of permutation equivariant layers. Permutation symmetry turns out to be closely tied to tensor contractions. That would allow us to synthesize efficient high-order permutation equivariant layers automatically in a procedural manner.
Finally, we'll discuss further optimizations that helps practical implementation. 

\paragraph{Common types of permutation symmetry.}

In the following table we analyze a few common problems by their type of permutation symmetry.

\begin{table}
\begin{tabular}{ c c c c }
\hline
 Problem       & Illustration  & Symmetry type  & Dependency \\
\hline
\begin{minipage}{.35\textwidth}
Predicting important weights to keep in a linear layer while pruning. Equivariant to neuron permutations along input `a` and output `b`. 
\end{minipage}
& 
    \begin{minipage}{.25\textwidth}
      \includegraphics[width=\linewidth]{Images/SRI/ab.png}
    \end{minipage} & ab &            \\
\begin{minipage}{.35\textwidth}
Group classes by common misclassifications given confusion matrices. Equivariant to class permutations `a` which simultaneously permutes both axes.  
\end{minipage}
& 
    \begin{minipage}{.25\textwidth}
      \includegraphics[width=\linewidth]{Images/SRI/aa.png}
    \end{minipage}  & aa &            \\
\begin{minipage}{.35\textwidth}
  Predicting the winner given players' hands. Equivariant to permutation of player ID a. Invariant to permutation of suits c. Invariant to card reordering b for each player independently. No symmetry against card number H.
\end{minipage}
&
\begin{minipage}{.25\textwidth}
  \includegraphics[width=\linewidth]{Images/SRI/abcH.png}
\end{minipage}  & abcH &  a$\rightarrow$b \\
\hline
\end{tabular}
\caption{Common permutation symmetries and their symmetry type notations.}
\end{table}





To aid discussions, we use a custom notation to describe the specific type of permutation symmetry, to capture both the input shape and the unique permutation axes. We have multiple dimensions and joint permutations whose symmetry notations are straight forward. 
There's also a dependency aspect, which captures a concept of "list of different lists". 
A fully independent batch dimension \lstinline{Z} and a non-symmetric latent dimension \lstinline{H} may be added optionally.


\paragraph{Creating a permutation equivariant layer with einsum pooling.}

Across all types of permutation symmetry, as we learned in Section I through Taylor series, it turns out that tensor contractions are are all you need for parameterizing permutation invariant and equivariant layers, which can then be stacked into a deep network.

Intuitively, tensor contractions like

$$
Y_{ij}=\sum_k \sum_l X_{ik} X_{lk} X_{lj} 
$$

create a new tensor that has the same shape as the input while summing over unused dimensions. They achieve a permutation equivariant effect. And tensor contractions like

$$
y=\sum_i \sum_j \sum_k \sum_l X_{ik} X_{lk} X_{lj} 
$$

that sum over all dimensions achieve a permutation invariant effect. 

As the math equations can get quite long, we will use the einsum notation\footnote{\url{https://numpy.org/doc/stable/reference/generated/numpy.einsum.html}} which represents a tensor contraction using the indices involved. It is widely used across deep learning frameworks to denote tensor contractions. For example,

\begin{minted}[breaklines,frame=single]{python}
Y=einsum('Zik,Zlk,Zlj->Zij',X,X,X)
y=einsum('Zik,Zlk,Zlj->Z',X,X,X)
\end{minted}

Here a batch dimension Z is added to make sure the right hand side is not empty.  

\textbf{How to create an equivariant layer given permutation symmetry type from tensor contractions?}
Our answer is two fully connected layers with a pooling layer in between. 

Let us use a 1D + latent \lstinline{aH}-type equivariant constraint as an example to illustrate the design.

The Taylor Series parameterization up to order 2 is

\begin{minted}[breaklines,frame=single]{python}
Y_abH=einsum('a->ba',a_H)
     +einsum('ab,ca->cb',b0_HH,X_aH)
     +einsum('ab,ca->db',b1_HH,X_aH)
     +einsum('abc,da,db->dc',c0_HHH,X_aH,X_aH)
     +einsum('abc,da,db->ec',c1_HHH,X_aH,X_aH)
     +einsum('abc,da,eb->dc',c2_HHH,X_aH,X_aH)
     +einsum('abc,da,eb->fc',c3_HHH,X_aH,X_aH)
     +...
\end{minted}

We can immediately see that the order-1 terms have $H^2$ parameters and order-2 terms have $H^3$ parameters, which would naturally need a low-rank($=K$) treatment, such as

\begin{minted}[breaklines,frame=single]{python}
Y_abH=einsum('a->ba',a_H)
     +einsum('ka,kb,ca->cb',b0U_KH,b0V_KH,X_aH)
     +einsum('ka,kb,ca->db',b1U_KH,b1V_KH,X_aH)
     +einsum('ka,kb,kc,da,db->dc',c0U,c0V,c0W,X_aH,X_aH)
     +einsum('ka,kb,kc,da,db->ec',c1U,c1V,c1W,X_aH,X_aH)
     +einsum('ka,kb,kc,da,eb->dc',c2U,c2V,c2W,X_aH,X_aH)
     +einsum('ka,kb,kc,da,eb->fc',c3U,c3V,c3W,X_aH,X_aH)
     +...
\end{minted}


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Images/SRI/layer.png}
    \caption{Left: Low-rank decomposition of high order coefficients. Right: An equivariant einsum layer with two linear layers an einsum pooling in between, which is the result of moving low-rank coefficients into linear fan-in and fan-out layers.}
\label{fig:einnet_layer}
\end{figure}



We can move the order-0 parameters, as well as $U$, $V$, $W$ matrices into fully connected layers along $H$ that perform input preprocessing and output postprocessing. So the end result is two linear layers with pooling in between, and for pooling we need 

\begin{minted}[breaklines,frame=single]{python}
Y_abH_0V=einsum('ck->ck',X_aH_0U)
Y_abH_1V=einsum('ck->dk',X_aH_1U)
Y_abH_0W=einsum('dk,dk->dk',X_aH_0U,X_aH_0V)
Y_abH_1W=einsum('dk,dk->ek',X_aH_1U,X_aH_1V)
Y_abH_2W=einsum('dk,ek->dk',X_aH_2U,X_aH_2V)
Y_abH_3W=einsum('dk,ek->fk',X_aH_3U,X_aH_3V)
...
\end{minted}

Notice that \lstinline{dk,ek->fk} can be composed with \lstinline{ck->dk} for each operand individually, and then combine using \lstinline{dk,dk->dk}. As we can stack more layers, not all pooling operations are needed and less pooling operations would reduce network complexity. In fact, this might be a good point to step back and ask: \textbf{Given equivariance type, e.g. \lstinline{aH}, how can we identify the minimum yet sufficient set of pooling operations?}

The following recipe might be helpful for designing pooling operations given equivariance type in practice:

1) Enumerate all valid and unique einsum operations up to order-k that are compatible with the given equivariance type. For example \lstinline{einsum('ab,bc->ac',X_ab,X_ab)} is compatible with \lstinline{aa}-type equivariance, but not compatible with \lstinline{ab}-type equivariance. Also notice that \lstinline{ba,ac->bc} is the just a renaming of \lstinline{ab,bc->ac}. There is a graph homomorphism problem under the hood for listing unique einsum operations and interested readers can dig deeper.

2) Filter einsum operations based on dependency requirement of the given equivariance type. For example \lstinline{einsum('ab,cb->cb',X_ab,X_ab)} satisfy \lstinline{b->a} dependency but does not satisfy \lstinline{a->b} dependency for \lstinline{ab}-type equivariance.

3) Filter out order-2+ ``breakable'' operations that can be divided into two lower order terms with a simple pointwise multiplication. For example \lstinline{ab,cb,cd,ad->ad} can be divided into \lstinline{ab,cb,cd->ad} and \lstinline{ad->ad} which can the be put together with \lstinline{ab,ab->ab}, so it is not necessary as long as the lower order terms exist. 

4) Normalize the rotation of input/output terms. For example for \lstinline{aa}-type equivariance, \lstinline{ab,cb->ca} is not necessary because it can be achieved with \lstinline{ab,bc->ac}, through applying rotations \lstinline{ab->ba} on the input and output.

5) Remove order-2+ operations that expand new dimensions in the output term. For example \lstinline{ab,bc->ad} is redundant because it can be achieved through \lstinline{ab,bc->ac} followed by a dimension expansion operation \lstinline{ab->ac}.

An algorithm that properly de-duplicates through compositions remains to be developed. But after all the filtering listed here, there is usually a quite compact initial set of pooling operations for further optimizations.

The following is a quick lookup table of pooling operations for a few common equivariance types.


\begin{table}
\begin{tabular}{ c c c }
\hline
 Symmetry type & Order & Pooling operation(s) \\
\hline
 aH          & 1     & aH$\rightarrow$aH, aH$\rightarrow$bH  \\
               & 2     & aH,aH$\rightarrow$aH  \\
               & 3+    & No need  \\
\hline
 abH         & 1     & abH$\rightarrow$abH, abH$\rightarrow$cbH, abH$\rightarrow$acH \\
               & 2     & abH,abH$\rightarrow$abH \\
               & 3     & abH,cbH,cdH$\rightarrow$adH \\
               & 4     & No need \\
               & 5     & abH,acH,dbH,dcH,deH$\rightarrow$aeH, abH,acH,dbH,dcH,ecH$\rightarrow$ebH \\
\hline
 aaH         & 1     & abH$\rightarrow$abH,aaH$\rightarrow$aaH,abH$\rightarrow$baH,abH$\rightarrow$cbH \\
               & 2     & abH,bcH$\rightarrow$acH,abH,abH$\rightarrow$abH \\
               & 3+    & No need  \\
\hline
\end{tabular}
\caption{Common equivariance types and their required einsum pooling operations.}
\end{table}



\paragraph{Putting everything together: The equivariant Einsum network.}

With an equivariant layer, we can stack them to create a practical high capacity neural net that learns well. Let's apply the following recipe

1) Stacking multiple equivariant layer to create a deep network.

2) GELU nonlinearity between equivariant layers to add to the depth and create bottlenecks.

3) Residual connections for better optimization dynamics.

4) Average pooling to create invariant dimensions if the symmetry involves invariance. 

The result is an equivariant backbone as Figure~\ref{fig:einnet_layer}.


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Images/SRI/arch.png}
    \caption{Stacking multiple equivariant layers to create a practical high capacity network.}
\label{fig:einnet_layer}
\end{figure}



High order einsum operations can result in large values. One consideration in practice is how to normalize them to be in line with lower order terms. Our observation is that mean subtraction and standard deviation normalization seems to help learning, but further research is still needed to improve learning stability.

Another consideration in practice is einsum path optimization\footnote{\url{https://numpy.org/doc/stable/reference/generated/numpy.einsum_path.html}}. For example, the einsum string \lstinline{ab,dc,ae,ac,db->de} by default is programmed to be computed pairwise from left to right. By the third term, a large factor \lstinline{abcde} would be created and stress the memory. Instead, if we compute pairwise via path \lstinline{ab,db->ad}, \lstinline{ac,dc->ad}, \lstinline{ad,ad->ad} and \lstinline{ad,ae->de}, the largest intermediate factor would only be 2-dimensional and the computation can also be done much faster. For modeling complex higher-order interations under certain types of symmetries, large einsums may be unavoidable, and computing them might be an interesting compute challenge.

Putting it all together, here is a reference Pytorch implementation of an Equivariant Einsum Network that would served as the backbone, to be followed by averaging for dimensions that need invariance. 
\begin{minted}[breaklines,frame=single]{python}
import torch
import torch.nn as nn
import torch.nn.functional as F

#Implements minimal aH-type pooling
class einpool_a(nn.Module):
    fan_in=4
    fan_out=3
    ndims=1
    def forward(self,x_):
        x=x_.view(-1,*x_.shape[-2:]) # Apply pooling only to the last 2 dims, supposedly `aH`
        N,KH=x.shape[-3:]
        H=KH//self.fan_in
        x=x.split(H,dim=-1)
        y0=x[0]
        y1=x[1].mean(-2,keepdim=True).repeat(1,N,1)
        y2=x[2]*x[3]
        y=torch.cat((y0,y1,y2),dim=-1)
        y=y.view(*x_.shape[:-1],-1) #Recover original tensor shape
        return y

#Implements minimal aaH-type pooling
class einpool_aa(nn.Module):
    fan_in=8
    fan_out=6
    ndims=2
    def forward(self,x_):
        x=x_.view(-1,*x_.shape[-3:]) # Apply pooling only to the last 3 dims, supposedly `aaH`
        N,M,KH=x.shape[-3:]
        H=KH//self.fan_in
        xn=x.view(-1,N*M,KH)
        xn=F.normalize(xn-xn.mean(-2,keepdim=True), dim=-2,p=2,eps=1e-1).view(*x.shape)
        x=x.split(H,dim=-1)
        xn=xn.split(H,dim=-1)
        y0=x[0]
        y1=x[1].diagonal(dim1=-2,dim2=-3).diag_embed(dim1=-2,dim2=-3)
        y2=x[2].transpose(-2,-3)
        y3=x[3].mean(-2,keepdim=True).repeat(1,1,M,1)
        y4=x[4]*x[5]
        y5=torch.einsum('ZabH,ZbcH->ZacH',xn[6],x[7])
        y=torch.cat((y0,y1,y2,y3,y4,y5),dim=-1)
        y=y.view(*x_.shape[:-1],-1) #Recover original tensor shape
        return y


#Implements order-3 abH-type pooling
class einpool_ab(nn.Module):
    fan_in=8
    fan_out=5
    ndims=2
    def forward(self,x_):
        x=x_.view(-1,*x_.shape[-3:]) # Apply pooling only to the last 3 dims, supposedly `abH`
        N,M,KH=x.shape[-3:] 
        H=KH//self.fan_in
        xn=x.view(-1,N*M,KH)
        xn=F.normalize(xn-xn.mean(-2,keepdim=True), dim=-2,p=2,eps=1e-12).view(*x.shape)
        #xn=F.softmax(x.view(-1,N*M,KH),dim=-2).view(*x.shape)
        x=x.split(H,dim=-1)
        xn=xn.split(H,dim=-1)
        y0=x[0]
        y1=x[1].mean(-2,keepdim=True).repeat(1,1,M,1)
        y2=x[2].mean(-3,keepdim=True).repeat(1,N,1,1)
        y3=xn[3]*x[4]
        y4=torch.einsum('ZacH,ZbcH,ZadH->ZbdH',xn[5],xn[6],x[7])
        y=torch.cat((y0,y1,y2,y3,y4),dim=-1) #
        y=y.view(*x_.shape[:-1],-1) #Recover original tensor shape
        return y


#Equivariant EinNet layer
class einnet_layer(nn.Module):
    def __init__(self,ninput,nh0,noutput,pool):
        super().__init__()
        self.fan_in=nn.Linear(ninput,nh0*pool.fan_in)
        self.fan_out=nn.Linear(nh0*pool.fan_out,noutput)
        self.pool=pool
    
    def forward(self,x):
        h=self.fan_in(x)
        h=self.pool(h)
        return self.fan_out(h)

#Equivariant EinNet backbone
class einnet(nn.Module):
    def __init__(self,ninput,nh0,nh,noutput,nstacks,pool):
        super().__init__()
        self.t=nn.ModuleList()
        self.t.append(einnet_layer(ninput,nh0,nh,pool))
        for i in range(nstacks-1):
            self.t.append(einnet_layer(nh,nh0,nh,pool))
        
        self.t.append(einnet_layer(nh,nh0,noutput,pool))
        self.pool=pool
    
    # Forward call
    #    x: tensor shape matches equivariance type, e.g. *abH
    def forward(self,x):
        h=self.t[0](x)
        for i in range(1,len(self.t)-1):
            h=h+self.t[i](F.gelu(h))
        
        return self.t[-1](F.gelu(h))

#Example usage
#    net=einnet(1,16,64,1,2,einpool_ab())
\end{minted}




